GPUReplay: A 50-KB GPU Stack for Client ML

GPUReplay (GR) is a novel way for deploying GPU-accelerated computation on mobile and embedded devices. It addresses high complexity of a modern GPU stack for deployment ease and security. The idea is to record GPU executions on the full GPU stack ahead of time and replay the executions on new input at run time. We address key challenges towards making GR feasible, sound, and practical to use. The resultant replayer is a drop-in replacement of the original GPU stack. It is tiny (50 KB of executable), robust (replaying long executions without divergence), portable (running in a commodity OS, in TEE, and baremetal), and quick to launch (speeding up startup by up to two orders of magnitude). We show that GPUReplay works with a variety of integrated GPU hardware, GPU APIs, ML frameworks, and 33 neural network (NN) implementations for inference or training. The code is available at https://github.com/bakhi/GPUReplay.

==> algo-replay.tex <==
% !TeX root = main.tex

\begin{comment}
\begin{algorithm}
	\caption{Replay}
	\begin{algorithmic}[1]
\WHILE{$IOIO_{next}$}
	\STATE ts, reg\_io = Interpret(\textit{IOIR})
	\STATE delay\_us = ts - prev\_ts
	\STATE {prev\_ts = ts}
	\STATE {Delay(delay\_us)}
	
	\IF{$IOIR_{job\_submission}$}
		\STATE {Sleep()}
	\ELSIF{$IOIR_{busywaiting}$}
		\REPEAT \STATE{val = Read\_reg($Reg\_addr$)} \UNTIL{val == expected\_value}
	\ELSE
		\STATE delay(delay\_us)
		\STATE Reg\_write() or Reg\_read()
	\ENDIF
	
	\STATE ...
\ENDWHILE
	\end{algorithmic}
\end{algorithm}
\end{comment}

\begin{algorithm}
	\caption{Replay}
	\begin{algorithmic}[1]
		\WHILE{\ir{}$_{next}$}
		\STATE \twait{}, RegIO = Interpret(\ir{})
		\STATE {Delay(\twait{})}
		
		\IF{$IOIR_{job\_submission}$}
		\STATE {Sleep()}
		\ELSIF{$IOIR_{busywaiting}$}
		\REPEAT \STATE{val = Read\_reg($Reg\_addr$)} \UNTIL{val == expected\_value}
		\ELSE
		\STATE RegIO
		\ENDIF
		
		\STATE ...
		
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}

==> discussion.tex <==
% !TeX root = main.tex

\section{Discussion}
\label{sec:discuss}

Things we can consider to discuss
\begin{itemize}
	\item Other GPU model (e.g. work with discrete GPUs such as nvidia)
\end{itemize}


==> fig-abs-model.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/abs-model} 
	%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
	\vspace{-5pt}		% use as needed
	\caption{The overview of the \sys{}. The \rec{} generates \ir{} which represents the abstract GPU model. Together with memory snapshot, \ir{} is transferred to the \rep{} in which the GPU computation is reproduced.}
	%\caption{The nondeterministic behavior of GPU and its software stack interaction}
	\label{fig:abs_model}
	\vspace{-8pt}		% use as needed
\end{figure}

==> fig-checkpoint.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth{}]{./figs/plot/over-checkpoint/over-checkpoint}
	\vspace{-5pt}		% use as needed
	\caption{Checkpoint overhead of each network. The memory copy is dominant factor of total execution time.}
	\label{fig:checkpoint}
	\vspace{-5pt}		% use as needed
\end{figure}

==> fig-cmp-design.tex <==
% !TeX root = main.tex

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/cmp} 
%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
%\vspace{-8pt}		% use as needed
\caption{The different ways to deploy a \sys{} replayer}
\label{fig:deployment}
%\vspace{-12pt}		% use as needed
\end{figure}

==> fig-delay.tex <==
% !TeX root = main.tex

\begin{figure*}
	\centering
	\subfloat[Mali G71]{
		\includegraphics[width=0.485\textwidth]{./figs/ml-infer-breakdown-mali}
	}
	\hfill
	\subfloat[v3d]{
		\includegraphics[width=0.485\textwidth]{./figs/ml-infer-breakdown-v3d}
	}
	\vspace{-5pt}
	\caption{NN inference delays. The replayer incurs similar delays as compared to the original GPU stack.}
	\label{fig:perf-ml-infer}
\end{figure*}

% 07/30/2021 heejin
% For ASPLOS template, subfigure doesn't work
\begin{comment}
\begin{figure*}
	\begin{subfigure}[b]{0.485\textwidth}
		\includegraphics[width=\textwidth]{./figs/ml-infer-breakdown-mali}
		\vspace{-14pt}		% use as needed
		\caption{Mali G71}
	\end{subfigure}
	~
	\hspace{3pt}
	\begin{subfigure}[b]{0.485\textwidth}
		\includegraphics[width=\textwidth]{./figs/ml-infer-breakdown-v3d}
		\vspace{-14pt}		% use as needed
		\caption{v3d}
	\end{subfigure}
	\vspace{-12pt}		% use as needed
	\caption{NN inference delays. The replayer incurs similar delays as compared to the original GPU stack.}
	\label{fig:perf-ml-infer}
	\vspace{-8pt}		% use as needed
\end{figure*}
\end{comment}

\begin{comment}
\begin{figure*}
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\begin{subfigure}[b]{0.182\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/mnist}
			%		\caption{MNIST}
		\end{subfigure}
		%\hspace{-2pt}
		%	~
		%	\begin{subfigure}[b]{0.075\textwidth}
		%		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/lenet}
		%		\vspace{-9pt}		% use as neededLeNet
		%%		\caption{LeNet}
		%	\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.157\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/alexnet}
			%		\caption{AlexNet}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.157\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/mobilenet}
			%		\caption{MobileNet}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.157\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/squeezenet}
			%		\caption{SqueezeNet}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.147\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/resnet12}
			%		\caption{ResNet12}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.147\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/vgg16}
			%		\caption{VGG16}
		\end{subfigure}
		
		\caption{ML inference with Mali Bifrost}
	\end{subfigure}
	\hspace{2pt}	
	~
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\begin{subfigure}[b]{0.175\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown-v3d/yolov4tiny}
			%		\caption{MNIST}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.15\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown-v3d/alexnet}
			%		\caption{AlexNet}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.15\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown-v3d/mobilenet}
			%		\caption{MobileNet}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.15\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown-v3d/squeezenet}
			%		\caption{SqueezeNet}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.15\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown-v3d/resnet18}
			%		\caption{ResNet12}
		\end{subfigure}
		\hspace{-2pt}
		~
		\begin{subfigure}[b]{0.15\textwidth}
			\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown-v3d/vgg16}
			%		\caption{VGG16}
		\end{subfigure}
		\caption{ML inference with v3d}
	\end{subfigure}
		\caption{Replay delays for NN inference, which are similar to those on the full GPU stack.}
%	\begin{itemize}
%		\item comp: the actual computation for inference (job running time)
%		\item mem: memory related including mem alloc, mmap, vmfault, etc.
%		\item user: Total delay - others
%		\item rec: recording time (measured in reality)
%		\item sched: interaction between user/kernel. e.g. user is waiting kernel event while doing FOPS\_POLL		
%		\item kernel: the time from user space pass the control to the device driver to the control is returned back to the user space. (e.g. IOCTL running time where the device driver does regIO, scheduling, etc)
%		\item model: overhead result from synchronized job submission
%		\item TS: TinyStack internal such as tuned delay between regI/O
%		
%	\end{itemize}
	\label{fig:perf-ml-infer}
	\vspace{-8pt}		% use as needed
\end{figure*}
\end{comment}

\begin{comment}


\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.075\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/mnist}
		\vspace{-9pt}		% use as needed
%		\caption{MNIST}
	\end{subfigure}
	\hspace{-2pt}
%	~
%	\begin{subfigure}[b]{0.075\textwidth}
%		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/lenet}
%		\vspace{-9pt}		% use as neededLeNet
%%		\caption{LeNet}
%	\end{subfigure}
%	\hspace{-2pt}
	~
	\begin{subfigure}[b]{0.08\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/alexnet}
		\vspace{-9pt}		% use as needed
%		\caption{AlexNet}
	\end{subfigure}
	\hspace{-2pt}
	~
	\begin{subfigure}[b]{0.08\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/mobilenet}
		\vspace{-9pt}		% use as needed
%		\caption{MobileNet}
	\end{subfigure}
	\hspace{-2pt}
	~
	\begin{subfigure}[b]{0.08\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/squeezenet}
		\vspace{-9pt}		% use as needed
%		\caption{SqueezeNet}
	\end{subfigure}
	\hspace{-2pt}
	~
	\begin{subfigure}[b]{0.08\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/resnet12}
		\vspace{-9pt}		% use as needed
%		\caption{ResNet12}
	\end{subfigure}
	\hspace{-2pt}
	~
	\begin{subfigure}[b]{0.08\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-infer-breakdown/vgg16}
		\vspace{-9pt}		% use as needed
%		\caption{VGG16}
	\end{subfigure}
	
	\vspace{-3pt}		% use as needed
	\caption{Inference delay distribution. After tuning the interval between replay actions, the \sys{} achieves comparable performance with the original execution with the full GPU stack.}
%	\begin{itemize}
%		\item comp: the actual computation for inference (job running time)
%		\item mem: memory related including mem alloc, mmap, vmfault, etc.
%		\item user: Total delay - others
%		\item rec: recording time (measured in reality)
%		\item sched: interaction between user/kernel. e.g. user is waiting kernel event while doing FOPS\_POLL		
%		\item kernel: the time from user space pass the control to the device driver to the control is returned back to the user space. (e.g. IOCTL running time where the device driver does regIO, scheduling, etc)
%		\item model: overhead result from synchronized job submission
%		\item TS: TinyStack internal such as tuned delay between regI/O
%		
%	\end{itemize}
	
	\label{fig:perf-ml-infer}
	
	\vspace{-8pt}		% use as needed
\end{figure*}

\end{comment}


==> fig-mmap.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth{}]{./figs/mmap} 
	%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
	\vspace{-5pt}		% use as needed
	\caption{A list of recording entries}
	%\caption{The nondeterministic behavior of GPU and its software stack interaction}
	\label{tab:ir}
	\vspace{-8pt}		% use as needed
\end{figure}

==> fig-motiv-ml-infer.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/motiv-ml-infer/alexNet}
		\vspace{-9pt}		% use as needed
		\caption{AlexNet}
	\end{subfigure}
	\hspace{6pt}
	~
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/motiv-ml-infer/mobileNet}
		\vspace{-9pt}		% use as needed
		\caption{MobileNet}
	\end{subfigure}

	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/motiv-ml-infer/alexNet_wo_prep}
		\vspace{-9pt}		% use as needed
		\caption{AlexNet w/o preparation}
	\end{subfigure}
	\hspace{6pt}
	~
	\begin{subfigure}[b]{0.22\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/motiv-ml-infer/mobileNet_wo_prep}
		\vspace{-9pt}		% use as needed
		\caption{MobileNet w/o preparation}

	\end{subfigure}
	\caption{Execution breakdown of ML inference.}
	\label{fig:motiv-ml-infer}
\end{figure}

==> fig-nondeterminism.tex <==
% !TeX root = main.tex

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/nondeterminism} 
%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
\vspace{-5pt}		% use as needed
\caption{The nondeterministic behaviors of GPU and interaction with its device driver. The job submission and execution time vary by the delays, which affect execution flow (e.g. \# of IRQs and GPU power state transition).}
%\caption{The nondeterministic behavior of GPU and its software stack interaction}
\label{fig:nondeterminism}
\vspace{-8pt}		% use as needed
\end{figure}

==> fig-perf-ml-infer.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/plot/perf-ml-infer/perf-ml-infer}
	\vspace{-9pt}		% use as needed
	\caption{ML inference exec time. The \sys{} has only xx\% overhead...}
	\label{fig:perf-ml-infer}
	\vspace{-8pt}		% use as needed
\end{figure}

\begin{comment}
\begin{figure*}
\centering
\begin{subfigure}[b]{0.35\textwidth}
	\includegraphics[width=\textwidth{}]{./figs/plot/perf-ml-infer/perf-ml-infer}
	\vspace{-9pt}		% use as needed
	\caption{ML inference exec time. The \sys{} has only xx\% overhead...}
	\label{fig:perf-ml-infer}
	\vspace{-8pt}		% use as needed
\end{subfigure}
~
\begin{subfigure}[b]{0.55\textwidth}
	\includegraphics[width=\textwidth{}]{./figs/plot/delay/delay}
	\vspace{-9pt}		% use as needed
	\caption{Distribution of delays (normalized to the actual job exec time). The \sys{} reduces delays (app, rec) by register IO time calibration.}
	\label{fig:delay}
	\vspace{-8pt}		% use as needed
\end{subfigure}
	\caption{Performance and overhead of ML inference}
\end{figure*}
\end{comment}

==> fig-perf-multi.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/plot/perf-multi/perf-multi}
	\vspace{-8pt}		% use as needed
	\caption{Abstract GPU model overhead. (1 to 1 job and IRQ). The larger input size it has, the lower overhead we get. TODO: add ML inference \textbf{XXX move to motivation. have real data XXX}}
	\label{fig:perf-multi}
	\vspace{-8pt}		% use as needed
\end{figure}

==> fig-perf-single.tex <==
% !TeX root = main.tex

\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.43\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-startup/perf-ml-startup}
		\vspace{-9pt}		% use as needed
		\caption{Startup time before the actual inference computation. XXX can break down like Fig 12?? XX}
		\label{fig:perf-ml-startup}
	\end{subfigure}
	\hspace{6pt}
	~
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer/perf-ml-infer}
		\vspace{-9pt}		% use as needed
		\caption{The computation time for inference (No startup/prep)}
		\label{fig:perf-ml-infer}
	\end{subfigure}
	\caption{Performance comparison between full stack and \sys{}.}
%		Performance distribution of simple application with \textbf{ARM Mali G71} and \textbf{VideoCore IV}, each of which is implemented with diver GPU programming abstract with a single or a few number of compute jobs. Original: default setting (not with abstract model: turn off debugFS and keep default power policy)
	\label{fig:perf-ml}
\end{figure*}

\begin{comment}

\begin{figure*}	
	\centering
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer-all/mnist}
		\vspace{-9pt}		% use as needed
		\caption{MNIST}
	\end{subfigure}
	\hspace{6pt}
	~
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer-all/lenet}
		\vspace{-9pt}		% use as needed
		\caption{LeNet}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer-all/alexnet}
		\vspace{-9pt}		% use as needed
		\caption{AlexNet}
	\end{subfigure}

	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer-all/mobilenet}
		\vspace{-9pt}		% use as needed
		\caption{MobileNet}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer-all/squeezenet}
		\vspace{-9pt}		% use as needed
		\caption{SqueezeNet}
	\end{subfigure}
	\hspace{6pt}
	~
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer-all/resnet12}
		\vspace{-9pt}		% use as needed
		\caption{ResNet12}
	\end{subfigure}
	
	\begin{subfigure}[b]{0.3\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-ml-infer-all/vgg16}
		\vspace{-9pt}		% use as needed
		\caption{VGG16}
	\end{subfigure}

	\caption{Single startup plus recursive inference running}
	\label{fig:perf-ml-combined}
\end{figure*}
\end{comment}

\begin{comment}
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali-cl/mali-cl}
		\vspace{-9pt}		% use as needed
		\caption{\textbf{Mali Bifrost G71} with \textbf{OpenCL}}
	\end{subfigure}

	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali-cl/mali-cl}
		\vspace{-9pt}		% use as needed
		\caption{\textbf{Mali Bifrost G71} with \textbf{GLES}}
	\end{subfigure}

	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali-cl/mali-cl}
		\vspace{-9pt}		% use as needed
		\caption{\textbf{VideoCore IV} with \textbf{GLES}}
	\end{subfigure}
	\caption{Performance distribution of simple application with \textbf{ARM Mali G71} (up) and \textbf{VideoCore IV} (down), each of which is implemented with diver GPU programming abstract with a single or a few number of compute jobs.}
	\label{fig:perf-single}
\end{figure}
\end{comment}

\begin{comment}

\begin{figure*}
	%	\centering
	%	\includegraphics[width=0.45\textwidth{}]{./figs/plot/perf-single/perf-single-vc-va}
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/vc/vc-va}
		\vspace{-9pt}		% use as needed
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/vc/vc-vm}
		\vspace{-9pt}		% use as needed
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/vc/vc-sha}
		\vspace{-9pt}		% use as needed	
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/vc/vc-sgemm}
		\vspace{-9pt}		% use as needed	
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/vc/vc-conv}
		\vspace{-9pt}		% use as needed	
	\end{subfigure}
	
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali/mali-va}
		\vspace{-9pt}		% use as needed
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali/mali-vm}
		\vspace{-9pt}		% use as needed
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali/mali-sha}
		\vspace{-9pt}		% use as needed	
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali/mali-sgemm}
		\vspace{-9pt}		% use as needed	
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.20\textwidth}
		\includegraphics[width=\textwidth]{./figs/plot/perf-single/mali/mali-conv}
		\vspace{-9pt}		% use as needed	
	\end{subfigure}
	\caption{Performance distribution of simple application with \textbf{ARM Mali G71} (up) and \textbf{VideoCore IV} (down), each of which is implemented with diver GPU programming abstract with a single or a few number of compute jobs.}
	\label{fig:perf-single}
\end{figure*}

\end{comment}

==> fig-pgt.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/pgt} 
%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
\vspace{-5pt}		% use as needed
\caption{Reconstruct page table in TEE of target device. The target receives GPU page table and remap virtual memory address to secure physical memory}
\label{fig:pgt}
\vspace{-10pt}		% use as needed
\end{figure}

==> fig-replay.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth{}]{./figs/replay} 
%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
\vspace{-5pt}		% use as needed
\caption{Replaying consists of two phase:1) preparation and 2) running.}
\label{fig:replay}
\vspace{-8pt}		% use as needed
\end{figure}

==> fig-symbol-inout.tex <==
% !TeX root = main.tex

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/symbol-inout} 
	%\missingfigure[figwidth=6cm]{Juno platform power instrumentation}
	\vspace{-5pt}		% use as needed
	\caption{symbol-based in/output address identification and dynamic memory snapshots. \textbf{can be merged with Fig. 6}}
	%\caption{The nondeterministic behavior of GPU and its software stack interaction}
	\label{fig:mmap}
	\vspace{-8pt}		% use as needed
\end{figure}

==> list-IR.tex <==
% !TeX root = main.tex

% ref: https://tex.stackexchange.com/questions/144170/lstlistings-reference-to-line-number
%\vspace{-1mm}
\lstset{
	language=C++,
	%	basicstyle=\ttfamily\footnotesize\small,
	basicstyle=\fontsize{8}{8}\selectfont\ttfamily,
	%	xleftmargin=5.0ex,
	%	framexleftmargin=5.0ex,
	frame=tb, % top & bottom
	breaklines=true,
	captionpos=b,
	%	numbers=left,
	label=list:ir-example}
\begin{lstlisting}[caption={Sample IR extracted from raw records.}, escapechar=!]
/* 1. Init: memory allocation */
map_region(0xffff6800, 4096);
map_region(0xffff8800, 16384)

/* 2. Replay */
reg_write(0us, JOB_IRQ_MASK, 0xffffffff);
reg_write(10us, JOB_IRQ_CLEAN, 0xffffffff);
reg_write(20us, MMU_UPDATE_REG, 0xffff8800);
reg_read_until(MMU_STATUS, 0x1);
reg_write(30us, JOB_SUBMIT_REG, 0xffff6800);
wait_irq() // pause replaying until IRQ arrives
reg_write(10us, JOB_IRQ_CLEAN, 0xffffffff);

/* 3. Term: mem free */
free_region(0xffff6800);
free_region(0xffff8800);
\end{lstlisting}
\vspace{-2mm}
% uint32_t sort(x_addr *dests, uint32_t n_outputs, x_addr src, idx_t keypos, idx_t reclen);

==> mem_manager.tex <==
% !TeX root = main.tex

\section{Memory Manager}
\label{sec:mem_manager}

\jin{intermediate stage of RnR which allocate all the memory and copies memory contents from snapshot to the proper location}

The \mm{} is in charge of intermediate stage of RnR. It prepares required memory space and reconstruct page table for replaying GPU running.

Before replaying, 

\mm{} prepares required memory space and reconstruct page table, which will be reflected to the GPU MMU.

\subsection{Memory allocation and copy snapshot}

The \mm{} allocates secure memory, decodes the snapshot and copies memory contents into the newly allocated memory.

\subsection{Page table reconstruction}
\jin{page table should be reconstructed using a newly allocated pages. reason: device's memory layout is different from each other}

\subsection{Put input and Get output}

\subsection{Remap the base address register of GPU}

\input{fig-pgt}

==> motiv.tex <==
% !TeX root = main.tex

\section{Background \& Motivation}
\label{sec:motiv}

==> record.tex <==
% !TeX root = main.tex

\section{Recording}
\label{sec:design}

\subsection{Register IO}

The GPU compute code passes through a large GPU software stack including both user space runtime and kernel space device driver. The user space runtime loads the GPU kernel source code and generates GPU job chain. it then communicates with device driver via ioctl (syscall) and enables the device driver to initiate GPU context and allocate necessary resources (e.g. GPU memory).
After constructing GPU page table and updating GPU MMU, the device driver submit the GPU job chain. Note that all the communication between device driver and GPU is completed via register read and write. For these reasons, we first record register read and write.

What we can do through register read and write are context initialization and termination, hardware interrupt handle, job submit, MMU update, and cache flush.

The benefits of register IO recording are as follows.

\begin{itemize}
	\item supporting a diverse GPU software stack. (e.g. OCL))
	\item no need of device driver.
\end{itemize}

\subsection{Necessary Resources}

\jin{page table, job chain}

Beside register read and write, we should record some more information which is created by device driver. The driver is in charge of constructing and updating GPU page table. It also submit the job delivered by user space driver to the GPU via register write. As GPU software stack is not in the TEE by our design choice, we somehow need to record all these information. To this end, \sys add one abstract layer inside device driver. It monitors user-device communication and record the job chain when user runtime submits it.

==> replay.tex <==
% !TeX root = main.tex

\section{Replay}
\label{sec:design}

\subsection{How to replay? - Loop}

\subsection{Interrupt Handler}

\subsection{MMIO Lockdown}



==> tab-cmp.tex <==
% !TeX root = main.tex
\begin{center}
	\fontsize{8.0}{9.0}\selectfont
	\setlength\tabcolsep{7pt}	% hp table insidem margin
	\begin{table}[h]
		\begin{tabular}{
%			@{}l@{$\;\;$}p{1mm}	% System
			l	% System
			l	% TEE
			l	% GPU stack in TEE
			c	% H/W Mod
			l	% SG
			}
			% <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
			\cellcolor{lightgray}\textbf{System} &
			\cellcolor{lightgray}\textbf{TEE} &
			\cellcolor{lightgray}\textbf{Stack in TEE} &
			\cellcolor{lightgray}\textbf{H/W Mod} &
			\cellcolor{lightgray}\textbf{SG} \jin{fix it}
			\\ 

			Slalom~\cite{slalom}
				& SGX
				& User
				& No
				& \texttt{CI-A-} \\

			Graviton~\cite{graviton}
				& SGX
				& User
				& Yes
				& \texttt{CI-A-} \\

			HIX\cite{hix}
				& SGX
				& User, Kernel
				& Yes
				& \texttt{CI-A-} \\
	
			Telekine\cite{telekine}
				& SGX
				& None (from client)
				& Yes
				& \texttt{CI-A-} \\
	
			HETEE\cite{HETEE}
				& SGX
				& User, Kernel
				& Yes
				& \texttt{CI-A-} \\

			\sys{}
				& TZ
				& None
			& No
			& \texttt{CI-A-} \\
			
			% \hlineB{2.5}
			%Glamdring~\cite{glamdring}	 	 & stream			& SGX	& n/a\\
			\end{tabular}
		\fontsize{7}{7}\selectfont
		\textbf{SG}: security guarantees. \\ %  N/R: not reported.
%		\textbf{MT}: support for multithreading within one TEE. \\
		\texttt{C}: data confidentiality; 
		\texttt{I}: data integrity;  
		\texttt{V}: verifiability; 
		\texttt{A}: analytics confidentiality;
		\texttt{O}: obliviousness \\
%		\vspace{-3mm}
		\caption{Comparison to existing secure GPU execution \textbf{this is fine. But can we draw a few system diagrams showing the difference?}}
%		\vspace{-2mm}
		\label{tab:cmp}
	\end{table}
\end{center}


==> tab-src.tex <==
% !TeX root = main.tex

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{center}
\begin{table}[]
	\centering
	\fontsize{8.0}{9.0}\selectfont
	\begin{tabular}{c c c c}
		\hline
		\rowcolor[HTML]{a5e6a5}
		\hlineB{1.5}
		\textbf{Record (Mali)} & \textbf{Replay (User)} & \textbf{Replay (kmod)} & \textbf{Total} \\ \hline
		0.7K & 2.2K & 0.7K & 3.6K (xxx)           \\ \hline
		\hlineB{1.5}
	\end{tabular}
	
	\vspace{3pt}		% use as needed
	\caption{A source code break down of the \sys{}. Binary code sizes shown in parentheses.}
	\label{tab:src}
	\vspace{-10pt}		% use as needed

\end{table}
\end{center}

==> tab-trace.tex <==
% !TeX root = main.tex

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{center}
\begin{table}[]
	\centering
	\fontsize{7}{8}\selectfont
	\begin{tabular}{l V{3} c c c c}
		\hline
		\rowcolor[HTML]{F0EE47} 
			\hlineB{1.5}
			\textbf{Benchmarks}  & \textbf{\texttt{job\_start}} & \textbf{\texttt{reg\_write}} & \textbf{\texttt{reg\_poll}} & \textbf{Total} \\ \hline
			\hlineB{1.5}
			\textbf{VecAdd (VA)}			& 1		& 200 	& xx	& xx \\
			\textbf{Scale (SC)}				& 5		& 300 	& xx	& xx \\
			\textbf{AbsDiff (AD)}			& 1		& 200 	& xx	& xx \\
			\textbf{DirectConv (DC)}		& 5		& 300 	& xx	& xx \\
			\textbf{MatrixConv (MC)}		& 5		& 300 	& xx	& xx \\
			\textbf{SGEMM (MM)}				& 7		& 600 	& xx	& xx \\
			\textbf{MNIST}					& 10	& 1000	& xx	& xx \\
			\textbf{ResNet}					& 20	& 2000	& xx	& xx \\
			\textbf{MobileNet}				& 80	& 8000	& xx	& xx \\
			\textbf{AlexNet}				& 56	& 5000	& xx	& xx \\
			\hlineB{1.5}
	\end{tabular}
	\vspace{3pt}		% use as needed
	\caption{IR break down of each benchmarks.}
	\label{tab:bnech}
	\vspace{-10pt}		% use as needed

\end{table}
\end{center}

==> threat_model.tex <==
% !TeX root = main.tex

%\section{Threat Model \& Security Approach}
%\label{sec:threat_model}


\begin{comment}

\paragraph{In-scope threats}
We do not trust replayer's normal world application at all as we assume a powerful adversary who takes a full control of system including a whole GPU software stack and OS kernel. The adversary can modify user space GPU runtime which may corrupt GPU computation or generate an unintentional result. The adversary can also inject some malicious code among GPU compute pipeline so that she can sniff the user's private information.
By compromising GPU scheduler in the device driver, the attacker can delay the GPU execution or exchange the user submitted compute job with the compromised one. This is possible as the adversary can know the actual input/output address via examining GPU page table in the driver.
We trust both i) developer's system environment including GPU stack and ii) TEE on the target device and the code running on it. We assume a secure boot of TEE, which guarantees the integrity of TEE code when loaded.

\paragraph{Out-of-scope threats}
\Note{merge, or go to evaluation}
We do not shield the following attacks: i) physical attacks such as cold boot or bus snooping; ii) power side-channel (the attacker may know power consumed by secure GPU execution); iii) physical attacks such as cold boot or bus snooping; \jin{think obliviousness, side channel (timing side channel).
\end{comment}


\jin{move here to merge}
\textbf{threat model - single purpose device}	
In such scenario, we assume the OS kernel is trustworthy and the adversary is unprivileged and hence, she cannot escalate privilege by exploiting vulnerabilities in the system stack. However, we assume the vulnerabilities in GPU software stack is as is and hence, she can modify user space GPU runtime which may corrupt GPU computation or generate unintentional result (compromising computation correctness). Besides, she is able to sniff the secret from non-zeroed memory after the computation.

\textbf{threat model - background compute GPU-shared device}
In this scenario, we do not trust all the client's applications in the REE and assume a much more powerful attacker than before, who can take a full control of system including a whole GPU software stack and OS kernel.
Including the previous threats, the adversary can inject some malicious code among GPU compute pipeline so that she can steal the user's private information.
By compromising GPU scheduler in the device driver, the adversary can delay the GPU execution or exchange the user submitted compute job with the compromised one. This is possible as the adversary can know the actual in/output addresses via carefully examining GPU page table in the driver.
We trust both i) developer's system environment including GPU stack and ii) TEE on the target device and the code running on it. We assume a secure boot of TEE, which guarantees the integrity of TEE code when loaded.


\paragraph{In-scope threats}
We do not trust replayer's normal world application at all as we assume a powerful adversary who takes a full control of system including a whole GPU software stack and OS kernel. The adversary can modify user space GPU runtime which may corrupt GPU computation or generate an unintentional result. The adversary can also inject some malicious code among GPU compute pipeline so that she can sniff the user's private information.
By compromising GPU scheduler in the device driver, the attacker can delay the GPU execution or exchange the user submitted compute job with the compromised one. This is possible as the adversary can know the actual input/output address via examining GPU page table in the driver.
We trust both i) developer's system environment including GPU stack and ii) TEE on the target device and the code running on it. We assume a secure boot of TEE, which guarantees the integrity of TEE code when loaded.

\Note{move to security analysis}
Note that we do not shield the following attacks: i) physical attacks such as cold boot or bus snooping; ii) power side-channel (the attacker may know power consumed by secure GPU execution); iii) physical attacks such as cold boot or bus snooping; \jin{think obliviousness, side channel (timing side channel)}

\begin{comment}
To this end, there are several ways to protect GPU execution: i) porting partial or entire GPU software stack into CPU TEE; ii) using lightweight homomorphic encryption with GPU computation and verifying the result within TEE.
However, porting GPU software stack requires additional effort as the GPU software stack is diverse, large and complicated which even results in a large TCB size that is possibly menace the entire TEE. In addition, homomorhpic encryption is functionally limited and incurs additional overhead which is even more critical to the mobile environment. Note that this approach cannot avoid porting partial GPU software stack as well.
\end{comment}

==> todo.tex <==
% !TeX root = main.tex

%\jin{Should we stress on mobile GPU?} - yes. or embedded GPU. 

% \jin{How to describe ML training result? Federated and transfer learning}
%\Note{explain GPU memory}

%\Note{integrated GPUs ... keep reminding}

%\Note{shader}

%\jin{fine-tune figures (e.g. bold), revise related works, revisit HIX, Graviton, Telekine, HETEE}

%\Note{text formating}
